FairProof : Confidential and Certifiable Fairness for Neural Networks

Machine learning models are increasingly used in societal applications, yet legal and privacy concerns demand that they very often be kept confidential. Consequently, there is a growing distrust about the fairness properties of these models in the minds of consumers, who are often at the receiving end of model predictions. To this end, we propose \name -- a system that uses Zero-Knowledge Proofs (a cryptographic primitive) to publicly verify the fairness of a model, while maintaining confidentiality. We also propose a fairness certification algorithm for fully-connected neural networks which is befitting to ZKPs and is used in this system. We implement \name in Gnark and demonstrate empirically that our system is practically feasible. Code is available at https://github.com/infinite-pursuits/FairProof.

==> extra.tex <==



%Since a facet can be shared by only two polytopes,  at most one of these neighboring polytopes has not yet been explored. If such a
polytope exists, for each of its facets, the algorithm computes the distance and inserts the facet into the
priority queue, and also add this new polytope to the set of explored polytopes. At initialization, the set of seen polytopes is composed only of the polytope containing $x$ and 





For neural networks, this boils down to solving the following optimization problem\begin{equation}
    \min_{x \in \B} ||x-\x||_2
\end{equation}
where $\B$ denotes the boundary of the polyhedral complex obtained from  $\m$ containing $\x$. 




\noindent\textbf{Algorithm.}
In this section, we describe the concrete algorithm to compute the local individiual fairness parameter for a data point $\x$ (Algorithm \ref{alg:IF}). 
Our construction is based on the Geocert algorithm by Jordan et. al (Algorithm \ref{alg:geo}, Section \ref{sec:background:PLNN}) for computing the pointwise $\ell_2$ robustness of neural networks with two key distinctions. First, we run on all the union of $(n-k)$-dimensional polytopes each of which corresponds to a fixed value of the sensitive feature set $\S$. Second, for each of these complices, we compute a lower bound on the pointwise $\ell_2$ robustness. The final certificate of fairness is the minimum over all the above bounds. 

In the following, we describe the working of the algorithm in more detail. 
 First, we compute the polyhedral complex $\PC_{\m}$ for the model $\m$ (Step 1). Next for a fixed value of the set of the sensitive features $\S$ (Step 3), we compute the corresponding $(n-k)$-dimensional polyhedral complex $\PC'$ from the original $n$-dimensional polyhedral complex (Steps 4-9). The key idea is to fix the corresponding values of the features in $\S$ in the linear constraints of the polytopes in $\PC_\m$. We provide an illustrative example in Appendix \ref{app:background}. In the next step, we compute a lower bound on the pointwise $\ell_2$ robustness of $\x$ for the polyhedral complex $\PC'$ using the Geocert algorithm (Step 10-11). In particular, instead of minimizing the $\ell_2$ distance to a facet $\F$, we compute the projection of $\x$ onto a hyperplane $H$, where $\F$ lies entirely on $H$. The above computation is repeated for all the values of the set of sensitive features $\S$. The final certificate of fairness is the minimum of all the lower bounds as computed above (Step 14).  



 In what follows, we briefly describe how to compute of the pointwise $\ell_2$ robustness of a point $x$. The problem essentially boils down to computing the largest $\ell_2$ ball centered at $x$ that fits within the union of n-dimensional polytopes defined by $f$. 





 %Finally, unlike any prior work, our individual fairness certificationenables a \textit{personalized} certificate for each prediction. We argue that in our specific commercial  context, where a user obtains a model prediction from $\m$ as a service, such an individualized fairness certificate is more valuable for the user. In this scenario, it is reasonable to assume that a user would be more concerned about the fairness of the model w.r.t to their data point (for example, how similar is the loan approval decision in its neighborhood) rather than  a one-size-fits-all global guarantee on the entire model. 
\begin{comment}\noindent\textbf{Problem statement.} Consider a model owner who wants  to use a model $\m$ for a classification task and provide a ML-as-a-Service (MLaaS) platform for users. The model is confidential and cannot be released publicly. A user $\U$ can obtain a classification on their data point $x$ via only an API access to $\m$.  However, the model owner still wants to be able to provide a certification of fairness, $\C$, of $\m$ for $\U$ w.r.t to their data point $\x$ -- the certificate $\C$ can be verified for its correctness.
Specifically, our goal here is two fold:
\begin{itemize}
    \item \textbf{Uniformity.} The model owner \textit{commits} to a model $\m$ that will be applied uniformly for everyone. In other words, the commitment ensures that the \textit{same} model $\m$ is used for classifying \textit{every} data point.
    \item \textbf{Certified individual fairness guarantee.} The model itself satisfies some individual fairness guarantee for the data point $x$. Specifically (based on Def. \ref{def:IF} and our aforementioned assumptions, $\m$ is $\epsilon$-individually fair w.r.t a data point $\x$ iff, 
    \begin{equation}
    \forall x, \forall S \in \mathcal{S},  \thinspace (x(S)=\x(S) \wedge  ||x-\x||_2\leq \epsilon ) \implies \m(\x)=\m(x)\label{eq:IF} 
    \end{equation}
Intuitively this means that the model's classification is independent of the sensitive features $\S$ within a $\ell_2$ ball centered at the data point $x$. In other words, the model $\m$ is \textit{fair} in its classification for the data points that are in the neighborhood of $x$. 
\end{itemize}
While uniformity can be achieved using prior work (such as, function commitment schemes ~\cite{Boneh21}), we are the first to provide both the aforementioned properties for  neural networks. 


Thus in our setting, the model owner acts as the prover and the user $\U$ acts as the verifer (see Sec. \ref{sec:background:ZKP}). The program $P$ evaluates to 1 iff, 
\begin{itemize}
    \item $y==\m(x)$, and 
    \item $\m$ is $\epsilon$-IF w.r.t $x$ \end{itemize}
\end{comment}




















%This is more setting where a user obtains a model prediction from $\m$ as a service. 
    

    
    
   %In the typical auditing setting, the goal is to audit the model and analyze its global fairness property. For instance, in case the measure of fairness is IF, a model $\m$ is defined to be $\epsilon_G$- globally IF if it is $\epsilon_G$-locally IF for \textit{all} data points $x\sim \D$. Instead here, we consider a commercial MLaaS setting where a user obtains a model prediction from $\m$ as a service. We argue that in this setting an individualized certificate of fairness (such as local IF guarantee as in Def. \ref{def:IF})) is more lucrative for the user and the reason is as follows. First, given IF as the chosen metric for fairness, it is reasonable to assume that an individual user would be more concerned about how fair the model was w.r.t to their data point (i.e. how similar are the predictions in its neighborhood)  as opposed to a global IF property. Additionally, note that the global IF guarantee $\epsilon_G$ is the minimum over all the individual local IF guarantees.  Hence, giving a local IF guarantee would be more informative for an user -- more often than not $\epsilon>\epsilon_G$ where $\epsilon$ is the local IF parameter, thereby giving the user higher confidence in the fairness of the model w.r.t. to their data. 
 
    
%We bypass this requirement through ZKP. 

%In contrast in our setting, the model owner can issue the certificate by directly analyzing the model weights and architecture. Thus, such a white-box certification mechanism gives more flexibility. Note that the black-box as discussed above can be performed complimentarily to our certification mechanism by simply querying $\m$. 


%In our setting, the bank owner is the prover while the client. The progrm is that P(w)=  


%Recall that certifying individual fairness in our setting entails computing the local individual fairness parameter for a given data point $x$, i.e., the certificate $\C$ is just the parameter $\epsilon$ (Def. \ref{def:IF}). Our mechanism is based on the following two key technical ideas.


%In this section, we describe our mechanism for certifying individual fairness in cleartext. We defer the relevant discussion on how to generate a ZKP for verifying the individual fairness certificate in the following section.  


%Our choice of the certification mechanism is based on  two reasons. First, the proposed mechanism satisfies our desiderata as mentioned in Section \ref{sec:certification}. Secondly, the mechanism is amenable to efficient verification using ZKPs (see the following section for more details). 



\begin{comment}Formally, the certifiable individual fairness problem can be expressed as:
 \begin{gather*}\epsilon = \min_{x\in \B} ||x-\x ||_2 \\\text{s.t. }
\langle x-\x,e_\S\rangle=0 \end{gather*}
where $e_\S$ has an $1$ for all the indices corresponding to the sensitive features in $\S$ and a $0$ in all the other $n-k$ indices.
\end{comment}






\begin{comment}\begin{table*}[ht]
  \centering
  \smallskip
  \scalebox{0.9}{
  \begin{tabular}{l|c|c|c|c|c|c|c|r}
    \hline
    \multirow{2}{*}{Dataset-Model} & \multicolumn{2}{c|}{VerifyPolytope} & \multicolumn{2}{c|}{VerifyDistance} & \multicolumn{2}{c|}{VerifyBoundary} & \multicolumn{2}{c}{VerifyInference} \\
    \cline{2-9}
    & Prove & Verify & Prove & Verify & Prove & Verify & Prove & Verify\\
    \toprule
    German [4,2] & 57.77 (13.83) & 0.157 (0.2) & 41.36 (14.71) & 1.23 (0.65) & 4.58 (6.1) & 0.03 (0.08) & 1.23 (0.53) & 0.035 (0.08)\\
     \hline
    German [8,2] & 62.42 (20.73) & 0.16 (0.28) & 225 (119) & 6.8 (3.8) & 11.15 (6.24) & 0.1 (0.18) & 1.16 (0.51) & 0.03 (0.08) \\
    
    \midrule

    Credit [4,2] & 50.12 (10.8) & 0.16 (0.21) & 29.82 (8.39) & 0.93 (0.48) & 6.48 (5.57) & 0.06 (0.11) & 1.035 (0.44) & 0.03 (0.06) \\
    
    \hline

    Credit [8,2] & 55.07 (11.35) & 0.12 (0.17) & 159.11 (97.5) & 4.6 (3) & 0.83 (2.58) & 0.007 (0.03) & 1.12 (0.43) & 0.03 (0.07) \\
    
    \midrule

    Adult [4,2] & 25.68 (6.21) & 0.23 (0.37) & 35.34 (10.94) & 1.15 (0.64) & 4.17 (4.8) & 0.04 (0.09) & 1.10 (0.39) & 0.52 (0.86) \\
    \hline
    Adult [8,2] & 15.75 (4.4) & 0.12 (0.15) & 46.23 (20.52) & 1.39 (0.73) & 5.51 (2.78) & 0.04 (0.07) & 0.63 (0.34) & 0.02 (0.05) \\
    \bottomrule
    \end{tabular}}
      \caption{\label{tb3:dtexptab} Proving and verification timings (in seconds) for various circuits, estimated by randomly sampling 100 test points for each dataset and model.}
\end{table*}

\end{comment}

\begin{comment}
\begin{table}
\centering
\begin{tabular}{lrr}
\hline
 Metric           &      Avg &      Std    \\
\hline
 Time (ms)            &  37.3045 & 3.82665               \\
 \#Facet            & 934.07   & 5.64669               \\
 \#Polytopes & 148.1    & 0.714143  \\
$\epsilon$          &  37.5291 & 1.34393               \\
\hline
\end{tabular}
\caption{Statistics for \textit{Credit}} \label{tab:credit:fair}
\end{table}
\begin{table}
\centering
\begin{tabular}{lrr}
\hline
 Metric           &      Avg &      Std \\
\hline
 Time (ms)             &  35.2267 & 3.49628   \\
 \#Facet            & 905.84   & 4.8841   \\
 \#Polytopes & 144      & 0        \\
$\epsilon$          & 261.057  & 0.783811  \\
\hline
\end{tabular}
\caption{Statistics for \textit{Adult}}\label{tab:adult:fair}
\end{table}
\begin{table}
\centering
\begin{tabular}{lrr}
\hline
 Metric           &       Avg &        Std \\
\hline
 Time (ms)             &  36.1164  &  14.1865   \\
 \#Facet            & 913.59    & 387.238     \\
 \#Polytopes & 145.49    &  65.6036   \\
 $\epsilon$          &   2.46221 &   0.744084 \\
\hline
\end{tabular}
\caption{Statistics for \textit{German}}\label{tab:german:fair}
\end{table}

\end{comment}
\begin{comment}
\begin{table*}[ht]
  \centering
  \smallskip
  \scalebox{0.8}{
  \begin{tabular}{l|c|c|c|c|c|c|c|c|c|r}
    \hline
    \multirow{2}{*}{Dataset-Model} & \multicolumn{2}{c|}{VerifyNeighbor} & \multicolumn{2}{c|}{VerifyNormalFacet} & \multicolumn{2}{c|}{VerifyMakeAdvConst} & \multicolumn{2}{c|}{VerifyOrder} & \multicolumn{2}{c}{VerifyMin} \\
    \cline{2-11}
    & Prove & Verify & Prove & Verify & Prove & Verify & Prove (min) & Verify & Prove & Verify \\
    \toprule
    
    German [4,2] & 0.21 (0.12) & 0.001 (8e-4) & 169.24 (75.58) & 1.45 (0.84) & 1.67 (0.77) & 0.47 (0.44) & 0.27 (0.15) & 0.07 (0.05) & 0.387 (0.28) & 0.009 (0.03)\\
     \hline
     German [8,2] & 0.88 (0.51) & 0.004 (0.002) & 574 (389) & 5.22 (3.72) & 5.67 (2.99) & 1.74 (1.29) & 7.76 (6.94) & 0.37 (0.34) & 0.37 (0.31)&0.009 (0.03) \\
    \midrule
    
    Credit [4,2] & 0.13 (0.06) & 6e-4 (5e-4) & 106 (52) & 0.89 (0.71) & 1.06 (0.55) & 0.38 (0.41)  & 0.25 (0.1) & 0.07 (0.05) & 0.38 (0.24) &0.003 (0.007)\\
    \hline
    Credit [8,2] & 0.62 (0.42) & 0.003 (0.002) & 1082 (405) & 9.15 (3.89) & 3.7 (2.42) & 1.2 (1.04) & 5.83 (5.41) & 0.32 (0.34) & 0.41 (0.3) & 0.006 (0.013)\\
    
    \midrule

    Adult [4,2] & 0.09 (0.04) & 7e-4 (6e-4) & 131.52 (47.71) & 1.27 (0.76) & 1.17 (0.66) & 0.36 (0.37) & 0.52 (0.3) & 0.08 (0.06) & 0.37 (0.27) &0.006 (0.01)\\
    
    \hline
    Adult [8,2] & 0.08 (0.05) & 5e-4 (4e-4) & 53.63 (49.15) & 0.5 (0.53) & 0.81 (0.53) & 0.3 (0.24) & 1.93 (1.83)& 0.1 (0.11) & 0.24 (0.17) &0.003 (0.004)\\
    \bottomrule
    
    \end{tabular}}
      \caption{\label{tb3:dtexptab} Proving and verification timings (in seconds) for various circuits, estimated by randomly sampling 100 test points for each dataset and model.}
\end{table*}
\end{comment}


\begin{comment}\begin{table*}[ht]
  \centering
  \smallskip
  \scalebox{0.7}{
  \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
    \hline
    Dataset-Model & VerifyPolytope & VerifyDistance & VerifyBoundary & VerifyInference & VerifyNeighbor & VerifyNormalFacet & VerifyMakeAdvConst & VerifyOrder & VerifyMin \\
    \toprule
    German [4,2] & 2.18 (9e-4) & 34.5 (19.2) & 0.9 (1.04) & 1.09 (6e-4) & 15 (11.56) & 30.47 (19.73) & 6.09 (3.85) & 8.12 (6.81) & 0.54 (4e-4) \\
     \hline 

    German [8,2] & 2.18 (9e-4) & 253 (297) & 1.98 (0.52) & 1.09 (7e-4) & 89.34 (121) & 161 (264) & 30.87 (40.5) & 45.56 (47.60) & 0.54 (5e-4) \\
    \midrule

    Credit [4,2] & 2.18 (9e-4) & 27.42 (14) & 1.36 (0.9) & 1.09 (6e-4) & 10.62 (8) & 20 (13.2) & 4.63 (2.67) & 6.97 (4.61) & 0.54 (4e-4) \\

    \hline

    Credit [8,2] & 2.18 (0.001) & 168.45 (205) & 0.24 (0.6) & 1.09 (8e-4) & 55.86 (81.58) & 250.28 (255.8) & 19.71 (27.2) & 37.37 (52.41) & 0.54 (4e-4) \\
    
    \midrule

    Adult [4,2] & 2.17 (8e-4) & 31.06 (19.55) & 0.91 (0.85) & 1.08 (7e-4) & 13.03 (11.87) & 31.37 (24.59) & 5.43 (3.95)& 7.91 (7.13) & 0.54 (4e-4) \\
    
    \hline
    Adult [8,2] & 2.18 (0.001) & 93.76 (108) & 2.18 (9e-4) & 1.08 (6e-4) & 28.25 (40.89) & 40.52 (82.3) & 10.5 (13.63) & 18.76 (29.46) & 0.54 (5e-4) \\
    \bottomrule

    
    \end{tabular}}
      \caption{\label{tb3:dtexptab} Proof Sizes (in KiloBytes) for various circuits, estimated by randomly sampling 100 test points for each dataset and model.}
\end{table*}
\end{comment}


\begin{comment}
    \begin{table*}[ht]
  \centering
  \smallskip
  \scalebox{0.65}{
  \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|r}
    \hline
    \multirow{2}{*}{Dataset-Model} & \multicolumn{2}{c|}{VerifyPolytope} & \multicolumn{2}{c|}{VerifyBoundary} & \multicolumn{2}{c|}{VerifyNeighbor} & \multicolumn{2}{c|}{VerifyDistance} & \multicolumn{2}{c|}{VerifyOrder} & \multicolumn{2}{c}{VerifyMin}\\
    \cline{2-13}
    & Prove (m) & Verify (s) & Prove (m) & Verify (s) & Prove (m) & Verify (s) & Prove (m) & Verify (s) & Prove (m) & Verify (s) & Prove (m) & Verify (s) \\
    \toprule
    German [4,2] & 1.00 (0.23) & 0.18 (0.21) & 2.91 (1.23) & 1.43 (0.81) & 3.63 (1.97) & 1.63 (1.07) & 0.69 (0.24) & 1.26 (0.67) & 0.27 (0.14) & 0.07 (0.05) & 0.006 (0.004) & 0.008 (0.03) \\
    %German [4,2] & 0.21 (0.12) & 0.001 (8e-4) & 169.24 (75.58) & 1.45 (0.84) & 1.67 (0.77) & 0.47 (0.44) & 0.27 (0.15) & 0.07 (0.05) & 0.387 (0.28) & 0.009 (0.03)\\
     \hline
     %German [8,2] & 0.88 (0.51) & 0.004 (0.002) & 574 (389) & 5.22 (3.72) & 5.67 (2.99) & 1.74 (1.29) & 7.76 (6.94) & 0.37 (0.34) & 0.37 (0.31)&0.009 (0.03) \\

     German [2,4] & 0.42 (0.11) & 0.11 (0.17) & 0.48 (0.18) & 0.17 (0.16) & 0.67 (0.31) & 0.23 (0.22) & 0.23 (0.06) & 0.25  (0.17) & 0.02 (0.01) & 0.01 (0.009) & 0.003 (0.002) & 0.003 (0.005) \\
     
    \midrule
    
    %Credit [4,2] & 0.13 (0.06) & 6e-4 (5e-4) & 106 (52) & 0.89 (0.71) & 1.06 (0.55) & 0.38 (0.41)  & 0.25 (0.1) & 0.07 (0.05) & 0.38 (0.24) &0.003 (0.007)\\
    Credit [4,2] & 0.85 (0.18) & 0.20 (0.23) & 1.89 (0.81) & 0.95 (0.69) & 2.33 (1.09) & 1.03 (0.70) & 0.50 (0.14) & 0.95 (0.47) & 0.26 (0.11) & 0.07 (0.06) & 0.006 (0.004) & 0.008 (0.04) \\
    \hline
    %Credit [8,2] & 0.62 (0.42) & 0.003 (0.002) & 1082 (405) & 9.15 (3.89) & 3.7 (2.42) & 1.2 (1.04) & 5.83 (5.41) & 0.32 (0.34) & 0.41 (0.3) & 0.006 (0.013)\\
    Credit [2,4] & 0.61 (0.12) & 0.26 (0.31) & 1.06 (0.40) & 0.54 (0.37) & 1.12 (0.75) & 0.68 (0.68) & 0.32 (0.11) & 0.58 (0.35) & 0.08 (0.04) & 0.03 (0.02) & 0.005 (0.004) & 0.009 (0.03)\\ 
    
    \midrule

    %Adult [4,2] & 0.09 (0.04) & 7e-4 (6e-4) & 131.52 (47.71) & 1.27 (0.76) & 1.17 (0.66) & 0.36 (0.37) & 0.52 (0.3) & 0.08 (0.06) & 0.37 (0.27) &0.006 (0.01)\\
    Adult [4,2] & 0.44 (0.11) & 0.26 (0.37) & 2.33 (0.79) & 1.31 (0.74) & 1.74 (0.81) & 1.20 (0.80) & 0.62 (0.18) & 1.22 (0.62) & 0.53 (0.30) & 0.09 (0.06) & 0.006 (0.004) & 0.007 (0.02) \\
    \hline
    %Adult [8,2] & 0.08 (0.05) & 5e-4 (4e-4) & 53.63 (49.15) & 0.5 (0.53) & 0.81 (0.53) & 0.3 (0.24) & 1.93 (1.83)& 0.1 (0.11) & 0.24 (0.17) &0.003 (0.004)\\

    Adult [8,2] & 0.27 (0.08) & 0.15 (0.16) & 0.96 (0.74) & 0.53 (0.48) & 1.35 (0.80) & 0.83 (0.57) & 0.76 (0.33) & 1.37 (0.70) & 1.93 (1.90) & 0.10 (0.11) & 0.004 (0.003) & 0.003 (0.005)\\
    \bottomrule
    
    \end{tabular}}
      \caption{\label{tb3:dtexptab} Proving (in minutes) and verification (in seconds) timings for various circuits, estimated by randomly sampling 100 test points for each dataset and model.}
\end{table*}
\end{comment}
\begin{comment}
    \begin{table*}[ht]
  \centering
  \smallskip
  \scalebox{0.7}{
  \begin{tabular}{l|c|c|c|c|c|c}
    \hline
    Dataset-Model & VerifyPolytope & VerifyBoundary & VerifyNeighbor & VerifyDistance & VerifyOrder & VerifyMin \\
    \toprule
    %German [4,2] & 2.18 (9e-4) & 34.5 (19.2) & 0.9 (1.04) & 1.09 (6e-4) & 15 (11.56) & 30.47 (19.73) & 6.09 (3.85) & 8.12 (6.81) & 0.54 (4e-4) \\

    German [4,2] & 3.27 (0.001) & 31.25 (19.58) & 20.97 (15.33) & 34.35 (19.09) & 7.76 (5.86) & 0.55 (5e-4) \\
     \hline 

    %German [8,2] & 2.18 (9e-4) & 253 (297) & 1.98 (0.52) & 1.09 (7e-4) & 89.34 (121) & 161 (264) & 30.87 (40.5) & 45.56 (47.60) & 0.54 (5e-4) \\
    German [2,4] & 3.27 (0.001) & 7.96 (3.42) & 8.21 (4.65) & 18.12 (6.62) & 5.35 (2.92) & 0.54 (5e-4) \\
    \midrule

    %Credit [4,2] & 2.18 (9e-4) & 27.42 (14) & 1.36 (0.9) & 1.09 (6e-4) & 10.62 (8) & 20 (13.2) & 4.63 (2.67) & 6.97 (4.61) & 0.54 (4e-4) \\
    Credit [4,2] & 3.27 (0.001) & 21.75 (13.11) & 15.63 (10.63) & 27.93 (13.82) & 7.21 (5.34) & 0.55 (4e-4) \\

    \hline

    %Credit [8,2] & 2.18 (0.001) & 168.45 (205) & 0.24 (0.6) & 1.09 (8e-4) & 55.86 (81.58) & 250.28 (255.8) & 19.71 (27.2) & 37.37 (52.41) & 0.54 (4e-4) \\
    Credit [2,4] & 3.27 (0.001) & 12.79 (6.24) & 9.59 (6.58) & 19.87 (9.32) & 5.50 (2.95) & 0.54 (5e-4) \\
    
    \midrule

    %Adult [4,2] & 2.17 (8e-4) & 31.06 (19.55) & 0.91 (0.85) & 1.08 (7e-4) & 13.03 (11.87) & 31.37 (24.59) & 5.43 (3.95)& 7.91 (7.13) & 0.54 (4e-4) \\
    Adult [4,2] & 3.27 (0.001) & 34.63 (24.57) & 20.37 (16.02) & 33.51 (19.81) & 7.92 (7.14) & 0.54 (5e-4) \\
    
    \hline
    %Adult [8,2] & 2.18 (0.001) & 93.76 (108) & 2.18 (9e-4) & 1.08 (6e-4) & 28.25 (40.89) & 40.52 (82.3) & 10.5 (13.63) & 18.76 (29.46) & 0.54 (5e-4) \\
    Adult [8,2] & 3.27 (0.001) & 36.41 (58.74) & 35.15 (43.47) & 86.97 (88.39) & 18.20 (29.37) & 0.54 (5e-4) \\
    \bottomrule

    
    \end{tabular}}
      \caption{\label{tb3:dtexptab} Proof Sizes (in KiloBytes) for various circuits, estimated by randomly sampling 100 test points for each dataset and model.}
\end{table*}\end{comment}

==> model_fairness_chhavi.tex <==
The objective of the experiments described in this section is to evaluate whether IFCert can distinguish models of varying degrees of fairness. Ideally, on average the IF parameter $\epsilon$ for a fair model should be larger than that for an unfair model.
%For this, we use the individual fairness parameter as our  metric. 

As is known in the literature, overfitting leads to unfairer models and regularization has been suggested as a remedy to train fairer models \cite{islam2021can}. We enlist these observations to obtain typical and unfair models by training with and without regularization (problems - weight decay is very high). We vary regularization through the weight decay parameter in Pytorch.

We randomly sample 100 data points from the test set and find the corresponding IF parameter $\epsilon$ for both the typical and unfair models. As demonstrated in figures \ref{fig:unfair} and \ref{fig:fair}, the unfair models have a lower $\epsilon$ than the corresponding typical models. For instance, for German the regular model has $\epsilon=8.41$ while the unfair model has $\epsilon=0.41$.  Due to lack of space, the results for the other models are included in App. \ref{app:evaluation}.

%In Figs. \ref{fig:credit:fair}, \ref{fig:adult:fair} and \ref{fig:german:fair}, we report the distribution of the individual fairness parameter ($\epsilon$) for Credit, Adult and German, respectively, for the (2,4) model. For each dataset, we report our observations over 100 randomly sampled data points from the test set. We observe that \textit{Adult} has the highest value (mean $\epsilon$ = 20.26) while \textit{German} has the lowest (mean $\epsilon=$ 8.41). We illustrate how to interpret the values of $\epsilon$ with the following example. The \textit{German} dataset has features such as salary (values: 0 if no known salary; 1 if monthly salary <\$20K; 2 if monthly salary >\$20K) and housing (values: 0 if renting; 1 if owning; 2 if free housing). Consider two  data points -- $x_1$ for a non-foreign worker (sensitive feature) with salary >\$20K and free housing, and $x_2$ for a foreign worker with no reported salary, living in a rental, while all other features match with those of $x_1$. $\epsilon=10$ for $x_1$ implies that both the data points would get the same prediction for a loan application. 


%Next we investigate the efficacy of the individual fairness parameter as a metric for assessing fairness. For this we train separate models that are \textit{unfair} by design. Specifically, we train a overfitted model which results in bias in the predictions. We report our observations in Fig. \ref{fig:unfair}. We observe that the unfair models have a lower $\epsilon$ than the corresponding regular models. For instance, for German the regular model has $\epsilon=8.41$ while the unfair model has $\epsilon=0.41$.  Due to lack of space, the results for the other models are included in App. \ref{app:evaluation}.


%\textcolor{red}{Regularized model experiment} -- why regularization? hypothesis -- low regularization should lead to more overfitting and therefore smaller radii while opposite trend should be observed for higher values, reg is implemented via weight decay parameter in pytorch. we modify the value of weight decay to high and low, train different models with the same other parameters except this and plot the radii. 
%Additionally, we report some statistics of our certification mechanism in Table \ref{tab:stat}.



\begin{comment}\begin{itemize}
    \item Distribution of individual fairness parameter $\epsilon$ for a sample of 100 points
    \item Explain what $\epsilon$ means using illustrative examples -- mention that the features are standardized to fit $\mathcal{N}(0,1)$ normal distribution
    \item Plot values for an ``unfair" model and show how the $\epsilon$'s differ from a fair model
\end{itemize}
\end{comment}
